DragGaussian: Enabling Drag-style Manipulation on 3D Gaussian Representation

User-friendly 3D object editing is a challenging task that has attracted significant attention recently. The limitations of direct 3D object editing without 2D prior knowledge have prompted increased attention towards utilizing 2D generative models for 3D editing. While existing methods like Instruct NeRF-to-NeRF offer a solution, they often lack user-friendliness, particularly due to semantic guided editing. In the realm of 3D representation, 3D Gaussian Splatting emerges as a promising approach for its efficiency and natural explicit property, facilitating precise editing tasks. Building upon these insights, we propose DragGaussian, a 3D object drag-editing framework based on 3D Gaussian Splatting, leveraging diffusion models for interactive image editing with open-vocabulary input. This framework enables users to perform drag-based editing on pre-trained 3D Gaussian object models, producing modified 2D images through multi-view consistent editing. Our contributions include the introduction of a new task, the development of DragGaussian for interactive point-based 3D editing, and comprehensive validation of its effectiveness through qualitative and quantitative experiments.

==> acknowledgements.tex <==
\chapter*{Acknowledgments}
\addcontentsline{toc}{chapter}{Acknowledgments}

They say, graduation marks the crossing of countless mountains. Yet, I know the journey of research is long, with many more peaks lying ahead.

My first foray into research came under the guidance of an outstanding senior Yiyuan Zhang. During the early days of my third year, he urged me to read papers and listened to my PPT presentations. It was tough at the beginning, but I gradually progressed from reading just one paper a week to one per day. My formal initiation into research came in the second semester of my third year. The admirable and kind-hearted Professor Xinxiao Wu patiently discussed ideas with me, encouraging me to independently lead a project in the field of 3D computer vision. Through collaborative efforts with Zilin Zhu and Linqian Fan, and under the guidance of Harry, we overcame numerous obstacles and eventually achieved something. In the summer of 2023, I had the opportunity to join THU AIR, where under the guidance of Professor Hao Zhao and senior Beiwen Tian, I was introduced to some codes and theories in the field of Robotics, gaining insights into how academic achievements can be applied in the industry.

Upon my arrival in Chongqing in September 2023, I officially entered the gates of AIGC. The rapidly evolving and exciting research results filled me with excitement. With the patient guidance of Xingyi Yang, Qiuhong Shen, and Professor Xinchao Wang, I spent approximately two months reading numerous articles in the field of 3D generation and editing, finally gaining some understanding of this direction. Riding the wave of the 3D Gaussian trend, we proposed our first idea, only to find it had already been implemented by others in the second week. However, with the patience and guidance of my seniors, we eventually formulated a second idea, which became the topic of my thesis. During the winter break of 2024, my close friend Jing Xu, my classmate Yuheng Yuan, and I spent the holidays working overtime, discussing theories, conducting experiments, and developing UI. Although the outcome of this work was not as satisfactory as hoped, the theoretical knowledge gained and engineering skills honed throughout the process are deeply cherished.

Throughout my undergraduate and research careers, I am especially grateful to my parents. They have provided me with unwavering support both spiritually and materially. Countless nights when my experiments failed, my code wouldn't cooperate, or my ideas wouldn't come, they always sent me delicious food and encouraged me through video calls.

Professor Wu once told me, "To do research, one must first prepare mentally, remain focused, and have the courage to face challenges." General Secretary Xi Jinping once said, "Every outstanding person has a period of silent growth. That period is a time of great effort without immediate results, which we call 'rooting'." I believe pursuing a Ph.D. is a long journey of rooting in life. I hope to endure loneliness, remain focused, and one day see the blossoming of my efforts.

